Few-shot Weakly-Supervised Object Detection via Directional Statistics

Detecting novel objects from few examples has become an emerging topic in computer vision recently. However, these methods need fully annotated training images to learn new object categories which limits their applicability in real world scenarios such as field robotics. In this work, we propose a probabilistic multiple instance learning approach for few-shot Common Object Localization (COL) and few-shot Weakly Supervised Object Detection (WSOD). In these tasks, only image-level labels, which are much cheaper to acquire, are available. We find that operating on features extracted from the last layer of a pre-trained Faster-RCNN is more effective compared to previous episodic learning based few-shot COL methods. Our model simultaneously learns the distribution of the novel objects and localizes them via expectation-maximization steps. As a probabilistic model, we employ von Mises-Fisher (vMF) distribution which captures the semantic information better than Gaussian distribution when applied to the pre-trained embedding space. When the novel objects are localized, we utilize them to learn a linear appearance model to detect novel classes in new images. Our extensive experiments show that the proposed method, despite being simple, outperforms strong baselines in few-shot COL and WSOD, as well as large-scale WSOD tasks.

==> fig2.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/model.pdf}
\caption{\label{fig:model_summary} Summary of the proposed method. Each image is
represented by a bag of feature proposals in the embedding space. {\bf Common
Object Localization}: For each class (shown in distinctive color), the common
object representation $\btheta_c$ is estimated as within class weighted average
of proposals where the contribution of proposals are decided by their soft
labels. The soft labels represent the chance of proposals belonging to the
common class and are learned within a probabilistic framework via
expectation-maximization updates. The proposal with the highest soft label (most
likely to be the common class) is marked by plus sign ``+'' in each bag. {\bf
Object Detection}: A query feature $\xb$ is classified based on its distance to
all the class prototypes $\btheta_1$, $\btheta_2$, and $\btheta_3$. Background
class likelihood (not shown here) is employed to guide the common object
localization and object detection models.}
\end{center}
\end{figure}

